Information Flows in Encrypted Databases

In encrypted databases, sensitive data is protected from an untrusted server by encrypting columns using partially homomorphic encryption schemes, and storing encryption keys in a trusted client. However, encrypting columns and protecting encryption keys does not ensure confidentiality - sensitive data can leak during query processing due to information flows through the trusted client. In this paper, we propose SecureSQL, an encrypted database that partitions query processing between an untrusted server and a trusted client while ensuring the absence of information flows. Our evaluation based on OLTP benchmarks suggests that SecureSQL can protect against explicit flows with low overheads (< 30%). However, protecting against implicit flows can be expensive because it precludes the use of key databases optimizations and introduces additional round trips between client and server.

==> architecture.tex <==
\section{Architecture}

==> overview.tex <==
\section{Motivating example}
\label{sec:overview}
\begin{figure}[!t]	
\lstset{basicstyle=\ttfamily\scriptsize,tabsize=1,numbers=left,language=sql}
\lstinputlisting{motivating-example.sql}
\caption{
\label{fig:tpcc-payment-orig}
A T-SQL procedure derived from TPC-C}
\end{figure}

\begin{figure}[!t]	
\lstset{basicstyle=\ttfamily\scriptsize,tabsize=1,numbers=left,language=sql,xleftmargin=5ex}
\lstinputlisting{motivating-example-rewritten.sql}
\caption{
\label{fig:tpcc-payment-rewritten}
A rewritten stored procedure which is secure and preserves semantics.}
\end{figure}

Once we have ensured that there are no insecure information flows, we can partition the stored procedure using code transformations and support for distributed query processing in existing databases. 
Ideally, the partitioning must be efficient i.e. maximize the amount of computation on the server. 
In addition, the partitioning must preserve semantics, even when the stored procedure uses abstractions like transactions. 
In the running example, a partitioning much ensure that customer data is read and updated to both tables atomically. 

Clearly, these analyzes and transformations are complex, laborious and error-prone, especially for applications involving complex stored procedures and a large number of tables. 
The SecureSQL compiler automates analysis, code generation and key management, allowing developers to declaratively specify their security requirements and write the application as if the database was not encrypted.
%A few points to note about the rewriting. 
%First,  any code for managing keys in the shell database in automatically generated by the compiler (line 34). 
%Also observe the use of linked server (an abstraction for distributed query processing provided by most commercial databases) at lines 40 for executing queries and stored procedures against a remote data source. 
%Since the table reference in the query at line 9 points to a table on the server, the query optimizer on the client automatically partitions and executes the query on the server. 
%Finally, observe that the \sfif\ statement at line 33 has been completely offloaded to the server (in the form of a stored procedure at line 32) and replaced by a call to the stored procedure. 
%Our we support of series of optimizations that can offload multiple queries along with control flow logic to the server. 
%In this example, offloading the \sfif\ statement results in fewer round-trips when compared to rewriting where only individual queries are partitioned using linked server.                         

==> policy.tex <==

While our tool does not mandate a consistent encryption policy, our security guarantee is conditioned on consistency. 

